Block Edit Errors with Transpositions: Deterministic Document Exchange Protocols and Almost Optimal Binary Codes

Document exchange and error correcting codes are two fundamental problems regarding communications. In the first problem, Alice and Bob each holds a string, and the goal is for Alice to send a short sketch to Bob, so that Bob can recover Alice's string. In the second problem, Alice sends a message with some redundant information to Bob through a channel that can add adversarial errors, and the goal is for Bob to correctly recover the message despite the errors. In a recent work \cite{CJLW18}, the authors constructed explicit deterministic document exchange protocols and binary error correcting codes for edit errors with almost optimal parameters.\ Unfortunately, the constructions in \cite{CJLW18} do not work for other common errors such as block transpositions. In this paper, we generalize the constructions in \cite{CJLW18} to handle a much larger class of errors. These include bursts of insertions and deletions, as well as block transpositions. Specifically, we consider document exchange and error correcting codes where the total number of block insertions, block deletions, and block transpositions is at most $k \leq \alpha n/\log n$ for some constant $0<\alpha<1$. In addition, the total number of bits inserted and deleted by the first two kinds of operations is at most $t \leq \beta n$ for some constant $0<\beta<1$, where $n$ is the length of Alice's string or message. We construct explicit, deterministic document exchange protocols with sketch size $ O( (k \log n +t) \log^2 \frac{n}{k\log n + t} )$ and explicit binary error correcting code with $O(k \log n \log \log \log n+t)$ redundant bits.

==> intro2.tex <==
\section{Introduction}
In communications and more generally distributed computing environments, there often arise questions regarding the synchronization of files or messages. For example, a message sent from one party to another party through a channel may get modified by channel noise or adversarial errors, and files stored on distributed servers may become out of synch due to different edit operations by different users. In many situations, these questions can be formalized in the framework of the following two fundamental problems.

\begin{itemize}
\item \emph{Document exchange.} In this problem, two parties Alice and Bob each holds a string $x$ and $y$, and the two strings are within distance $k$ in some metric space. The goal is for Alice to send a short sketch to Bob, so that Bob can recover $x$ based on his string $y$ and the sketch. %Naturally, we would like to require both the message length and the computation time of Alice and Bob to be as small as possible.

\item \emph{Error correcting codes.} In this problem, two parties Alice and Bob are linked by a channel, which can change any string sent into another string within distance $k$ in some metric space. Alice's goal is to send a message to Bob. She does this by sending an encoding of the message with some redundancy information through the channel, so that Bob can recover the correct message despite any changes to the codeword. %Again, we would like to minimize both the codeword length (or equivalently, the number of redundant bits) and the encoding/decoding time. This is a generalization of the classical error correcting codes for Hamming errors.
\end{itemize}

These two problems are closely related. For example, in many cases a solution to the document exchange problem can also be used to construct an error correcting code, but the reverse direction is not necessarily true. In both problems, a major goal is to is to minimize the size of the sketch or the redundant information. For applications in computer science, we also require the computations of both parties to be efficient, i.e., in polynomial time of the input length. In this case we say that the solutions to these problems are \emph{explicit}. Here we focus on deterministic document exchange protocols and error correcting codes with a binary alphabet, arguably the most important setting in computer science.

Both problems have been studied extensively, but the known solutions and our knowledge vary significantly depending on the distance metric in these problems. In the case of Hamming distance (or Hamming errors),  we have explicit constructions with asymptotically optimal parameters. However, for other distance metric/error types, our understanding is still rather limited.

An important generalization of Hamming errors is edit errors, which consist of bit insertions and deletions. These are strictly more general than Hamming errors since a bit substitution can be replaced by a deletion followed by an insertion. Edit errors can happen in many practical situations, such as reading magnetic and optical media, mutations in gene sequences, and routing packets in internet protocols. However, these errors are considerably harder to handle, due to the fact that a single edit error can change all the indices of the bits in a string.

Non-explicitly, by using a greedy coloring algorithm or a sphere packing argument, one can show that the optimal size of the sketch in document exchange, or the redundant information in error correcting codes is roughly the same for both Hamming errors and edit errors. Specifically, suppose that Alice's string or message has length $n$ and the distance bound $k$ is relatively small (e.g., $k \leq n/4$), then for both Hamming errors and edit errors, the optimal size in both problems is $\Theta(k \log (\frac{n}{k}))$ \cite{Levenshtein66}. For Hamming errors, this can be achieved by using sophisticated linear Algebraic Geometric codes \cite{hoholdt1998algebraic}, but for edit errors the situation is quite different. We now describe some of the previous works regarding both document exchange and error correcting codes for edit errors.

\paragraph{Document exchange.} Orlitsky \cite{185373} first studied the document exchange problem for generally correlated strings $x, y$. Using the greedy graph coloring algorithm mentioned before, he obtained a deterministic protocol with sketch size $O(k \log n)$ for edit errors, but the running time is exponential in $k$. Subsequent improvements appeared in \cite{CormodePSV00}, \cite{irmak2005improved},  and \cite{Jowhari2012EfficientCP}, achieving sketch size $O(k \log(\frac{n}{k}) \log n)$ \cite{irmak2005improved} and $O(k \log^2 n \log^* n)$ \cite{Jowhari2012EfficientCP} with running time $\tilde{O}(n)$. A recent work by Chakraborty et al. \cite{Chakraborty2015LowDE} further obtained sketch size $O(k^2 \log n)$ and running time $\tilde{O}(n)$, by using a clever randomized embedding from the edit distance metric to the Hamming distance metric. Based on this work, Belazzougui and Zhang \cite{BelazzouguiZ16} gave an improved protocol with sketch size $O(k (\log^2 k+\log n))$,  which is asymptotically optimal for $k =2^{O(\sqrt{\log n})}$. The running time in \cite{BelazzouguiZ16} is $\tilde{O}(n+\poly(k))$.

Unfortunately, all of the above protocols, except the on in \cite{185373} which runs in exponential time, are randomized. Randomized protocols are less useful than deterministic ones in practice, and are also not suitable for the applications in constructing error correcting codes. However, designing an efficient deterministic protocol appears quite tricky, and it was not until 2015 when Belazzougui \cite{Belazzougui2015EfficientDS} gave the first protocol even for $k>1$. The protocol in \cite{Belazzougui2015EfficientDS} has sketch size $O(k^2 + k \log^2 n)$ and running time  $\tilde{O}(n)$.

\paragraph{Error correcting codes.} As fundamental objects in both theory and practice, error correcting codes have been studied extensively from the pioneering work of Shannon and Hamming. While great success has been achieved in constructing codes for Hamming errors, the progress on codes for edit errors has been quite slow despite much research. A work by Levenshtein \cite{Levenshtein66} in 1966 showed that the Varshamov-Tenengolts code \cite{VT65}  corrects one deletion with an optimal redundancy of roughly $\log n$ bits, but even correcting two deletions requires $\Omega(n)$ redundant bits. In 1999, Schulman and Zuckerman \cite{796406} gave an explicit asymptotically good code, that can correct up to $\Omega(n)$ edit errors with $O(n)$ redundant bits. However the same amount of redundancy is needed even for smaller number of errors. %and even the first explicit asymptotically good insdel code (a code that has constant rate and can also correct a constant fraction of insertion and deletion errors) over a constant alphabet did not appear until the work of  Schulman and Zuckerman in 1999 \cite{796406}, who gave such a code over the binary alphabet. We refer the reader to the survey by Mercier et al. \cite{MercierBT10} for more details about the extensive research on this topic.

For any fixed constant $k$, a recent work by Brakensiek et.\ al \cite{8022906} constructed an explicit code that can correct $k$ edit errors with $O(k^2 \log k \log n)$ redundant bits. This is asymptotically optimal when $k$ is a fixed constant, but the construction in \cite{8022906} only works for constant $k$, and breaks down for larger $k$ (e.g., $k=\log n$). Based on his deterministic document exchange protocol, Belazzougui \cite{Belazzougui2015EfficientDS} also gave an explicit code that can correct up to $k$ edit errors with $O(k^2 + k \log^2 n)$ redundant bits.

In a very recent work by the authors \cite{CJLW18}, we significantly improved the situation. Specifically, we constructed an explicit document exchange protocol with sketch size $O(k \log^2 \frac{n}{k}) $, which is optimal except for another $\log \frac{n}{k}$ factor. We also constructed explicit codes for $k$ edit errors with $O(k \log n)$ redundant bits, which is optimal for $k \leq n^{1-\alpha}$, any constant $0<\alpha<1$. These results bring our understanding of document exchange and error correcting codes for edit errors much closer to that of standard Hamming errors.

However, the constructions in \cite{CJLW18} do not work for other common types of errors, such as \emph{block transpositions}. Given any string $x$, a block transposition takes an arbitrary substring of $x$, moves it to a different position, and insert it into $x$. These errors happen frequently in distributed file systems and Internet protocols. For example, it is quite common that a user, when editing a file, copies a whole paragraph in the file and moves it to somewhere else; and in Internet routing protocols, packets can often get rearranged during the process. It is easy to see that even a single transposition of a block with length $t$ can result in $2t$ edit errors, thus a naive application of document exchange protocols or codes for edit errors will result in very bad parameters. 

In this paper we consider document exchange protocols and error correcting codes for edit errors as well as block transpositions. In fact, even for edit errors we also consider a larger, more general class of errors. Specifically, we consider edit errors that happen in \emph{bursts}. This kind of errors is also pretty common, as most errors that happen in practice, such as in wireless or mobile communications and magnetic disk readings, tend to be concentrated. We model such errors as \emph{block} insertions and deletions, where in one operation the adversary can insert or delete a substring of the original string. It is again easy to see that this is indeed a generalization of standard edit errors. However, in addition to the bound $k$ on such operations, we also need to put a bound on the total number of bits that the adversary can insert or delete, since otherwise the adversary can simply delete the whole string in one block deletion. Therefore, we model the adversary as follows.

\paragraph{Model of the adversary.} An adversary considered in this paper is allowed to perform two kinds of operations: block insertion/deletion and block transposition. The adversary is allowed to perform $k_1$ block insertions/deletions and $k_2$ block transpositions, such that $k_1+k_2 \leq k$ for a given parameter $k$. In addition, the total number of bits inserted/deleted by block insertions/deletions is at most $t$ for a given parameter $t$. We note that by the result of Schulman and Zuckerman \cite{796406}, to correct $\Omega(n/\log n)$ block transpositions one needs at least $\Omega(n)$ redundant bits. Thus we only consider $k \leq \beta n/\log n$ for some constant $0< \beta<1$. Similarly, we only consider $t \leq \alpha n$ for for some constant $0< \alpha<1$ since otherwise the adversary can simply delete the whole string.

In this model, we show in the appendix that non-explicitly, the information optimum for both the sketch size of document exchange, and the redundancy of error correcting codes, is $\Theta(k \log n+t)$. However, as far as we know, there are no known explicit deterministic document exchange protocols; and the only randomized protocol which can handle edit errors as well as block transpositions is the protocol of \cite{irmak2005improved}, that has sketch size $O(k \log(\frac{n}{k}) \log n)$. Similarly, the only previous explicit code that can handle edit errors as well as block transpositions is the work of Schulman and Zuckerman \cite{796406}, which needs $\Omega(n)$ redundant bits even to correct one block transposition. We note that both of these works however did not study edit errors that can allow block insertions/deletions.

\subsection{Our results}
In this paper we construct explicit deterministic document exchange protocols, and error correcting codes for the adversary discussed above. We have the following theorems.
\begin{theorem}
There exists an explicit, deterministic document exchange protocol with sketch size $O(k \log n \log \frac{n}{k+t }+ t) $, for an adversary who can perform at most $k$ block insertions/deletions and block transpositions, where the total number of bits inserted/deleted is at most $t$. %=k_1 + k_2$, for $(k_1, t)$ block-insertions/deletions and $k_2$ block-transpositions.
\end{theorem}

This is the first explicit, deterministic document exchange protocol for edit errors with block transpositions.\ The sketch size matches the randomized protocol of \cite{irmak2005improved}, and is optimal up to an extra $\log \frac{n}{k+t }$ factor. 

Next we have the following theorem of error correcting codes.

\begin{theorem}
There exists an explicit binary code with redundancy of $O(k\log n\log\log n+t)$, that can correct at most $k$ block insertions/deletions and block transpositions, where the total number of bits inserted/deleted is at most $t$.
\end{theorem}

This significantly improves the result in Schulman and Zuckerman \cite{796406}, which needs $\Omega(n)$ redundant bits even to correct one block transposition. The redundancy here is also optimal up to an extra $\log \log n$ factor.

 
